BoGraph: Structured Bayesian Optimization From Logs for Expensive Systems with Many Parameters

Current auto-tuning frameworks struggle with tuning computer systems configurations due to their large parameter space, complex interdependencies, and high evaluation cost. Utilizing probabilistic models, Structured Bayesian Optimization (SBO) has recently overcome these difficulties. SBO decomposes the parameter space by utilizing contextual information provided by system experts leading to fast convergence. However, the complexity of building probabilistic models has hindered its wider adoption. We propose BoAnon, a SBO framework that learns the system structure from its logs. BoAnon provides an API enabling experts to encode knowledge of the system as performance models or components dependency. BoAnon takes in the learned structure and transforms it into a probabilistic graph model. Then it applies the expert-provided knowledge to the graph to further contextualize the system behavior. BoAnon probabilistic graph allows the optimizer to find efficient configurations faster than other methods. We evaluate BoAnon via a hardware architecture search problem, achieving an improvement in energy-latency objectives ranging from $5-7$ x-factors improvement over the default architecture. With its novel contextual structure learning pipeline, BoAnon makes using SBO accessible for a wide range of other computer systems such as databases and stream processors.

==> sections/eval_soc_table.tex <==
\toprule
model               & log EDP                    & Latency (1/sec)           & Power (mWatts)             & Cycles                     & Power/Ops                & Area                     \\
\midrule

\textbf{\BoGraph{}} & ${\mathbf{8.12 \pm 0.28}}$ & $\mathbf{11.06 \pm 0.19}$ & $\mathbf{27.37 \pm 11.59}$ & $53082 \pm 10755$          & $\mathbf{0.65 \pm 0.28}$ & $\mathbf{3.54 \pm 2.06}$ \\
PBTTuner            & $9.39 \pm \text{NA}$       & $18.53 \pm \text{NA}$     & $34.92 \pm \text{NA}$      & $61193 \pm \text{NA}$      & $0.84 \pm \text{NA}$     & $6.10 \pm \text{NA}$     \\
DeepGP              & $10.14 \pm 0.27$           & $11.06 \pm 3.92$          & $203.15 \pm 46.34$         & $68225 \pm 11177$          & $4.86 \pm 1.11$          & $110.81 \pm 55.96$       \\
BoTorch             & $10.44 \pm 0.62$           & $11.06 \pm 3.90$          & $108.46 \pm 102.97$        & $73349 \pm 15352$          & $2.59 \pm 2.46$          & $54.90 \pm 29.93$        \\
Random              & $10.74 \pm 0.19$           & $18.32 \pm 4.81$          & $143.94 \pm 194.83$        & $\mathbf{32133 \pm 29749}$ & $3.44 \pm 4.66$          & $64.36 \pm 52.80$        \\
\midrule
Default             & $14.50 \pm 0$              & $94.80 \pm 0$             & $220.34 \pm 0$             & $62193 \pm 0$              & $5.13 \pm 0$             & $35.18 \pm 0$            \\
\bottomrule

==> sections/logs_sample.tex <==
\begin{Verbatim}[fontsize=\scriptsize, commandchars=\\\{\}, gobble=2]
  # number of prefetches that crossed the page
  system.\textcolor{red}{cpu}.icache.prefetcher.pfSpanPage 585236
  # Cycle average of tags in use
  system.\textcolor{red}{l2}.tags.tagsinuse 7674.850251
  # Total number of bytes read from DRAM
  system.\textcolor{red}{mem\_ctrls}.bytesReadDRAM  315136
  ... 1000 additional metric
\end{Verbatim}

==> sections/tables/stencil_perf.tex <==
\begin{table}
    \caption{
        \label{tab:stenci3d_perf}
        Best found optimization for stencil3d environment for each model configuration. The lower the EDP, cycles, and power the better.
    }
    \vskip 0.15in
    \begin{center}
        \begin{small}
            \begin{sc}
                \begin{tabular}{lrrrr}
                    \toprule
                    model   & log(EDP)       & Pwr(mW)        & Cycles         & Pwr/Op           \\
                    \midrule
                    BoGraph & \textbf{23.76} & \textbf{43.22} & 18204          & \textbf{0.88}(W) \\
                    Random  & 24.40          & 180.77         & 13147          & 3.68(W)          \\
                    SMAC    & 24.66          & 55.55          & 12779          & 1.13(W)          \\
                    BoTorch & 25.20          & 520.70         & \textbf{11212} & 10.61(W)         \\
                    DeepGP  & 25.71          & 654.23         & 14886          & 13.33(W)         \\
                    \midrule
                    Default & 29.15          & 341.17         & 115860         & 6.75(W)          \\
                    \bottomrule
                \end{tabular}
            \end{sc}
        \end{small}
    \end{center}
    \vskip -0.1in
\end{table}
